Coverage and Energy Analysis of Mobile Sensor Nodes in Obstructed Noisy Indoor Environment: A Voronoi Approach

The rapid deployment of wireless sensor network (WSN) poses the challenge of finding optimal locations for the network nodes, especially so in (i) unknown and (ii) obstacle-rich environments. This paper addresses this challenge with BISON (Bio-Inspired Self-Organizing Network), a variant of the Voronoi algorithm. In line with the scenario challenges, BISON nodes are restricted to (i) locally sensed as well as (ii) noisy information on the basis of which they move, avoid obstacles and connect with neighboring nodes. Performance is measured as (i) the percentage of area covered, (ii) the total distance traveled by the nodes, (iii) the cumulative energy consumption and (iv) the uniformity of nodes distribution. Obstacle constellations and noise levels are studied systematically and a collision-free recovery strategy for failing nodes is proposed. Results obtained from extensive simulations show the algorithm outperforming previously reported approaches in both, convergence speed, as well as deployment cost.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> TMC paper - arXiv.org Version/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> TMC paper - arXiv.org Version/diagram.tex <==
%%%
\begin{picture}(500,200)(-3, 0)
\linethickness{0.2mm}
%%
%% Bounding box - remove for final version
%%
%        \put(  0,  0){
%            \put(0,0){\line( 1, 0){50}}
%            \put(0,0){\line( 0, 1){50}}}
%        \put(500,  0){
%            \put(0,0){\line(-1, 0){50}}
%            \put(0,0){\line( 0, 1){50}}}
%        \put(  0,200){
%            \put(0,0){\line( 1, 0){50}}
%            \put(0,0){\line( 0,-1){50}}}
%        \put(500,200){
%            \put(0,0){\line(-1, 0){50}}
%            \put(0,0){\line( 0,-1){50}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Block
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Outer Box LARGE LEFT TOP
\put(  0,200){% this is the upper left corner of the outer box
    %%%% outer boxes
        \put(  0,   0){\line( 1, 0){180}}
        \put(  0, -80){\line( 1, 0){180}}
        \put(  0,   0){\line( 0,-1){ 80}}
        \put(180,   0){\line( 0,-1){ 80}}
    %%%% Text
    \put(  0,  0){
        \put(  3,-13) {\cite{15,16,21,36,37,42,46f} for}}
    %%%% inner box top left
    \put(  5,-45){
        \put(  0, 25){% set to height of the inner box
            \put( 8,-10) {Detecting holes}
            \put( 18,-20) {in coverage}}
        \put(  0,  25){\line( 0,-1){ 25}}
        \put( 80,  25){\line( 0,-1){ 25}}
        \put(  0,   0){\line( 1, 0){ 80}}
        \put( 80,  25){\line(-1, 0){ 80}}}
    %%%% inner box top right
    \put( 95,-45){
        \put(  0, 25){% set to height of the inner box
            \put(  3,-10) {Maintaining uni-}
            \put(  3,-20) {form distribution}}
        \put(  0,  25){\line( 0,-1){ 25}}
        \put( 80,  25){\line( 0,-1){ 25}}
        \put(  0,   0){\line( 1, 0){ 80}}
        \put( 80,  25){\line(-1, 0){ 80}}}
    %%%% inner box middle
    \put( 43, -75){
        \put(  0, 25){% set to height of the inner box
            \put( 13,-10) {Improving the }
            \put(  3,-20) {scheduling scheme}}
        \put(  0,  25){\line( 0,-1){ 25}}
        \put( 86,  25){\line( 0,-1){ 25}}
        \put(  0,   0){\line( 1, 0){ 86}}
        \put( 86,  25){\line(-1, 0){ 86}}}
        %%%%
        }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Block
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Outer Box LARGE LEFT BOTTOM
\put(  0,110){% this is the upper left corner of the outer box
    %%%% outer boxes
        \put(  0,   0){\line( 1, 0){180}}
        \put(  0, -90){\line( 1, 0){180}}
        \put(  0,   0){\line( 0,-1){ 90}}
        \put(180,   0){\line( 0,-1){ 90}}
    %%%% Text
    \put(  0,  0){
        \put(  3,-13) {Leads to \cite{40,41,48,39,42a,43}}
        \put(  3,-23) {\cite{44,45,46,56-0,56,72}}}
    %%%% inner box top left
    \put(  2,-30){
        \put(  17,-10) {\textbf{Maximising}}
        \put(  0,   0){\line( 0,-1){ 55}}
        \put( 86,   0){\line( 0,-1){ 55}}
        \put(  0,   0){\line( 1, 0){ 86}}
        \put( 86, -55){\line(-1, 0){ 86}}
        %%% Little box 1
        \put(  2,-15){
            \put(  17, -12) {\footnotesize{Area Coverage}}
            \put(  0,   0){\line( 0,-1){ 18}}
            \put( 82,   0){\line( 0,-1){ 18}}
            \put(  0,   0){\line( 1, 0){ 82}}
            \put( 82, -18){\line(-1, 0){ 82}}}
        %%% Little box 2
         \put(  2,-35){
            \put(  21, -12) {\footnotesize{Convergence}}
            \put(  0,   0){\line( 0,-1){ 18}}
            \put( 82,   0){\line( 0,-1){ 18}}
            \put(  0,   0){\line( 1, 0){ 82}}
            \put( 82, -18){\line(-1, 0){ 82}}}}
        %%%%%%%%%%%%%%%%%
    %%%% inner box top right
    \put( 92,-30){
        \put(  17,-10) {\textbf{Minimizing}}
        \put(  0,   0){\line( 0,-1){ 55}}
        \put( 86,   0){\line( 0,-1){ 55}}
        \put(  0,   0){\line( 1, 0){ 86}}
        \put( 86, -55){\line(-1, 0){ 86}}
        %%% Little box 1
        \put(  2,-15){
            \put(  9, -12) {\footnotesize{Energy consumption}}
            \put(  0,   0){\line( 0,-1){ 18}}
            \put( 82,   0){\line( 0,-1){ 18}}
            \put(  0,   0){\line( 1, 0){ 82}}
            \put( 82, -18){\line(-1, 0){ 82}}}
        %%% Little box 2
         \put(  2,-35){
            \put(  19, -8) {\footnotesize{Computational}}
            \put(  25,-15) {\footnotesize{complexity}}
            \put(  0,   0){\line( 0,-1){ 18}}
            \put( 82,   0){\line( 0,-1){ 18}}
            \put(  0,   0){\line( 1, 0){ 82}}
            \put( 82, -18){\line(-1, 0){ 82}}}}
        %%%%%%%%%%%%%%%%%
        }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Block
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Outer Box SMALL MIDDLE TOP
\put(200,170){% this is the lower left corner of the outer box
\linethickness{0.5mm}
    %%%% Text
    \put(  0, 30){% set to height of the outer box
        \put(  6,-13) {Voronoi diagrams in}
        \put(  12,-23) {WSN deployment}}
    %%%% outer boxes
    \put(  0,  0){
        \put(  0,  0){
            \put(0,0){\line( 1, 0){100}}
            \put(0,0){\line( 0, 1){ 30}}}
        \put(100,  0){
            \put(0,0){\line(-1, 0){100}}
            \put(0,0){\line( 0, 1){ 30}}}
        \put(  0, 30){
            \put(0,0){\line( 1, 0){100}}
            \put(0,0){\line( 0,-1){ 30}}}
        \put(100, 30){
            \put(0,0){\line(-1, 0){100}}
            \put(0,0){\line( 0,-1){ 30}}}}}
\linethickness{0.2mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Block
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Outer Box SMALL MIDDLE MIDDLE
\put(190,150){% this is the lower left corner of the outer box
    %%%% outer boxes
        \put(  0,   0){\line( 1, 0){120}}
        \put(  0,-143){\line( 1, 0){120}}
        \put(  0,   0){\line( 0,-1){143}}
        \put(120,   0){\line( 0,-1){143}}
    %%%% Text
    \put(  0,  0){
        \put(  3,-13) {Generated through \cite{16}}
        \put(  3,-23) {\cite{40, 41,38,39,44}}
        \put(  3,-33) {\cite{46f,46ba,46bb}}}
    %%%% Inner box
        \put(  2,-40){
        \put(  3,-10) {Intersection of neighbours'}
        \put( 11,-20) {perpendicular bisectors}
        \put(  0,   0){\line( 0,-1){ 70}}
        \put(116,   0){\line( 0,-1){ 70}}
        \put(  0,   0){\line( 1, 0){116}}
        \put(116, -70){\line(-1, 0){116}}
        %%% Little box 1
        \put(  2,-25){
            \put( 25, -8) {\footnotesize{Euclidean distance}}
            \put( 20,-15) {\footnotesize{(homogeneous nodes)}}
            \put(  0,   0){\line( 0,-1){ 18}}
            \put(112,   0){\line( 0,-1){ 18}}
            \put(  0,   0){\line( 1, 0){112}}
            \put(112, -18){\line(-1, 0){112}}}
        %%% Little box 2
         \put(  2,-45){
            \put( 26, -8) {\footnotesize{Laguerre distance}}
            \put( 20,-15) {\footnotesize{(heterogeneous node)}}
            \put(  0,   0){\line( 0,-1){ 18}}
            \put(112,   0){\line( 0,-1){ 18}}
            \put(  0,   0){\line( 1, 0){112}}
            \put(112, -18){\line(-1, 0){112}}}}
        %%%%%%%%%%%%%%%%%
        %%% Last Little box 
        \put(  5,-120){
            \put( 20, -8) {\footnotesize{Intersected with node's}}
            \put( 35,-15) {\footnotesize{sensing range}}
            \put(  0,   0){\line( 0,-1){ 18}}
            \put(112,   0){\line( 0,-1){ 18}}
            \put(  0,   0){\line( 1, 0){112}}
            \put(112, -18){\line(-1, 0){112}}}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Block
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Outer Box LARGE RIGHT TOP
\put(320,200){% this is the upper left corner of the outer box
    %%%% outer boxes
        \put(  0,   0){\line( 1, 0){180}}
        \put(  0,-110){\line( 1, 0){180}}
        \put(  0,   0){\line( 0,-1){110}}
        \put(180,   0){\line( 0,-1){110}}
    %%%% Text
    \put(  0,  0){
        \put(  3,-13) {Implemented on randomly distributed}
        \put(  3,-23) {homogeneous / heterogeneous nodes in}
%        \put(  3,-33) {known / unknown environments}}
        \put(  3,-33) {known / unknown environments in \cite{40}}
        \put(  2,-44) {\cite{41,42,44,45,46,46f,46ba,46bb}}}
    %%%% inner box top left
    \put(  2,-50){
        \put(  10,-10) {\textbf{Avoiding noise}}
        \put(  0,   0){\line( 0,-1){ 55}}
        \put( 86,   0){\line( 0,-1){ 55}}
        \put(  0,   0){\line( 1, 0){ 86}}
        \put( 86, -55){\line(-1, 0){ 86}}
        %%% Little box 1
        \put(  2,-15){
            \put(  22, -8) {\footnotesize{Addition of}}
            \put(  14,-15) {\footnotesize{random numbers}}
            \put(  0,   0){\line( 0,-1){ 18}}
            \put( 82,   0){\line( 0,-1){ 18}}
            \put(  0,   0){\line( 1, 0){ 82}}
            \put( 82, -18){\line(-1, 0){ 82}}}
        %%% Little box 2
         \put(  2,-35){
            \put(  25, -8) {\footnotesize{Pre-defined}}
            \put(  21,-15) {\footnotesize{anchor nodes}}
            \put(  0,   0){\line( 0,-1){ 18}}
            \put( 82,   0){\line( 0,-1){ 18}}
            \put(  0,   0){\line( 1, 0){ 82}}
            \put( 82, -18){\line(-1, 0){ 82}}}}
        %%%%%%%%%%%%%%%%%
    %%%% inner box top right
    \put( 92,-50){
        \put(  3,-10) {\textbf{Avoiding obstacles}}
        \put(  0,   0){\line( 0,-1){ 55}}
        \put( 86,   0){\line( 0,-1){ 55}}
        \put(  0,   0){\line( 1, 0){ 86}}
        \put( 86, -55){\line(-1, 0){ 86}}
        %%% Little box 1
        \put(  2,-15){
            \put(  15, -12) {\footnotesize{Repulsive force}}
            \put(  0,   0){\line( 0,-1){ 18}}
            \put( 82,   0){\line( 0,-1){ 18}}
            \put(  0,   0){\line( 1, 0){ 82}}
            \put( 82, -18){\line(-1, 0){ 82}}}
        %%% Little box 2
         \put(  2,-35){
            \put(  20, -8) {\footnotesize{Scanning the}}
            \put(  21,-15) {\footnotesize{entire region}}
            \put(  0,   0){\line( 0,-1){ 18}}
            \put( 82,   0){\line( 0,-1){ 18}}
            \put(  0,   0){\line( 1, 0){ 82}}
            \put( 82, -18){\line(-1, 0){ 82}}}}
        %%%%%%%%%%%%%%%%%
        }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Block
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Outer Box LARGE RIGHT BOTTOM
\put(320, 80){% this is the upper left corner of the outer box
    %%%% outer boxes
        \put(  0,   0){\line( 1, 0){180}}
        \put(  0, -80){\line( 1, 0){180}}
        \put(  0,   0){\line( 0,-1){ 80}}
        \put(180,   0){\line( 0,-1){ 80}}
    %%%% Text
    \put(  0,  0){
        \put(  3,-13) {Position \cite{16,40,38,39,44,46bb}}}
    %%%% inner box top
    \put(  5,-45){
        \put(  0, 25){% set to height of the inner box
            \put( 38,-10) {\textbf{Voronoi ploygonial}}
            \put( 28,-20) {edges, vertices, centroids}}
        \put(  0,  25){\line( 0,-1){ 25}}
        \put(170,  25){\line( 0,-1){ 25}}
        \put(  0,   0){\line( 1, 0){170}}
        \put(170,  25){\line(-1, 0){170}}}
    %%%% inner box bottom
    \put(  5,-75){
        \put(  0, 25){% set to height of the inner box
            \put( 5,-10) {\textbf{Voronoi edges'} midpoint intersection /}
            \put( 18,-20) {closest to the furthest point vertex}}
        \put(  0,  25){\line( 0,-1){ 25}}
        \put(170,  25){\line( 0,-1){ 25}}
        \put(  0,   0){\line( 1, 0){170}}
        \put(170,  25){\line(-1, 0){170}}}
        }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The Arrows
%%% from the main box
\put(185,180){\ensuremath{\Leftarrow}}
\put(246,157){\ensuremath{\Downarrow}}
\put(305,180){\ensuremath{\Rightarrow}}
%%% secondary arrows down
\put( 86,113){\ensuremath{\Downarrow}}
\put(246, 33){\ensuremath{\Downarrow}}
\put(405,83){\ensuremath{\Downarrow}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{picture}
%%%

